Semantic and Effective Communication for Remote Control Tasks with Dynamic Feature Compression

The coordination of robotic swarms and the remote wireless control of industrial systems are among the major use cases for 5G and beyond systems: in these cases, the massive amounts of sensory information that needs to be shared over the wireless medium can overload even high-capacity connections. Consequently, solving the effective communication problem by optimizing the transmission strategy to discard irrelevant information can provide a significant advantage, but is often a very complex task. In this work, we consider a prototypal system in which an observer must communicate its sensory data to an actor controlling a task (e.g., a mobile robot in a factory). We then model it as a remote Partially Observable Markov Decision Process (POMDP), considering the effect of adopting semantic and effective communication-oriented solutions on the overall system performance. We split the communication problem by considering an ensemble Vector Quantized Variational Autoencoder (VQ-VAE) encoding, and train a Deep Reinforcement Learning (DRL) agent to dynamically adapt the quantization level, considering both the current state of the environment and the memory of past messages. We tested the proposed approach on the well-known CartPole reference control problem, obtaining a significant performance increase over traditional approaches

==> sections/abstract.tex <==
\begin{abstract}
The coordination of robotic swarms and the remote wireless control of industrial systems are among the major use cases for 6G: in these cases, the massive amounts of sensory information that needs to be shared over the wireless medium can overload even high-capacity connections. Consequently, solving the \emph{effective communication} problem by optimizing the transmission strategy to discard irrelevant information can provide a significant advantage, but it is often a very complex task. In this work, we define a remote \gls{pomdp} model, in which an observer must communicate its sensory data to an actor controlling a task (e.g., a mobile robot in a factory), and considers the semantic and effective communication problems. We split the task by considering an ensemble \gls{vqvae} encoding, and train a \gls{drl} agent to dynamically adapt the quantization level, considering both the current state of the environment and the memory of past messages. Our simulations show that this scheme obtains a significant performance increase on the classic Cartpole problem.
\end{abstract}

\begin{IEEEkeywords}
Effective communication, Networked control, Semantic communication, Information bottleneck
\end{IEEEkeywords}

==> sections/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

In this work we have presented a dynamic feature compression scheme that can exploit an ensemble \gls{vqvae} to solve the semantic and effective communication problems. The dynamic scheme significantly outperforms fixed quantization, and can be trained automatically with limited feedback, as well as overcoming the limitations of emergent communication models, which are unable to deal with complex tasks.

A natural extension to the model is to consider more complex tasks and wider communication channels, corresponding to realistic control scenarios. Another interesting direction for future work is to consider a joint training of the actor and observer, or cases with partial information is available at both the transmitter and the receiver.

%or partial information scenarios in which the actor and observer each have part of the state information, and the communication needs to consider what the actor may already know from its own observations.

==> sections/intro_related.tex <==
\section{Introduction}
\label{sec:intro}

In the introduction to Shannon's seminal work on communication theory~\cite{shannon1949mathematical}, Warren Weaver defined a problem with three levels: classical information theory deals with Level A, or the technical problem, which concerns itself with the accurate and efficient transmission of data. However, if communication is oriented toward affecting an agent's action by communicating some information, there are two further levels to the problem: Level B, or the semantic problem, is to find the most effective way to convey the \emph{meaning} of the message, even when irrelevant details are lost or misunderstood, while Level C, also called the effectiveness problem, deals with the resulting behavior of the receiver: as long as the receiver takes the optimal decision, the effectiveness problem is solved, regardless of any differences in the received information.

While the Level B and C problems attracted limited attention for decades, the explosion of \gls{iiot} systems has drawn the research and industrial communities toward semantic communication~\cite{popovski2020semantic}, optimizing remote control processes under severe communication constraints beyond Shannon's limits on Level A performance~\cite{gunduz2022beyond}. In particular, the effectiveness problem is highly relevant to robotic applications, in which independent mobile robots, such as drones or rovers, must operate based on information from remote sensors. In this case the sensors and cameras act as the transmitter in a communication problem, while the robot is the receiver: by solving the Level C problem, the sensors can transmit the information that best directs the robot's actions toward the optimal policy~\cite{stavrou2022rate}. In the case of offloaded computation, the  robot is the transmitter, while the remote controller is the receiver, which must get the most relevant information to decide the control policy~\cite{wan2020cognitive}.

The rise of metrics taking the content of the message into account such as \gls{voi}~\cite{yates2020agesurvey} in communications represents an attempt to approach the problem in practical scenarios, and analytical studies have exploited information theory to define a semantic accuracy metric and minimize distortion~\cite{shao2022theory}. In particular, \emph{information bottleneck} theory~\cite{beck2022semantic} has been widely used to characterize Level B optimization~\cite{shao2021learning}. However, translating a practical system model into a semantic space is a non-trivial issue, and the semantic problem is a subject of active research~\cite{uysal2022semantic}.
The effectiveness problem is even more complex, as it represents a dual problem: communication needs to be optimized not only toward minimizing semantic distortion, but toward distortion in directions that affect the control policy in meaningful ways~\cite{tung2021effective}. While the effect of simple scheduling policies is relatively easy to compute~\cite{kim2019learning}, and linear control systems can be optimized explicitly~\cite{zheng2020urgency}, realistic control tasks are highly complex, complicating an analytical approach to the Level C problem. Pure learning-based solutions that consider communication as an action in a multi-agent \gls{drl} problem, such as emergent communication, also have limitations~\cite{foerster2016learning}, as they can only deal with very simple scenarios due to significant convergence and training issues. In some cases, the information bottleneck approach can also~\cite{goyal2018transfer} be exploited to determine state importance, but the existing literature on optimizing Level C communication is very sparse, and limited to simpler scenarios~\cite{rcmab_pase}.

In this work, we consider a dual model which combines concepts from \gls{drl} and semantic source coding: we consider an ensemble \gls{vqvae} model~\cite{van2017neural}, each of which learns to represent observations using a different codebook. A \gls{drl} agent can then select the codebook to be used for each transmission, controlling the trade-off between accuracy and compression. Depending on the task of the receiver, the reward to the \gls{drl} agent can be tuned to solve the Level A, B, and C problems, optimizing the performance for each specific task.
In order to test the performance of the proposed framework, we consider the well-known CartPole problem, whose state can be easily converted into a semantic space, as its dynamics depend on a limited set of physical quantities. We show that dynamic codebook selection outperforms static strategies for all three levels, and that considering the Level C task can significantly improve control performance with the same bitrate.

The rest of the paper is organized as follows: first, we present the general system model in Sec.~\ref{sec:system}. We then present the dynamic feature compression solution in Sec.~\ref{sec:solution}, which is evaluated by simulation in Sec.~\ref{sec:results}. Finally, Sec.~\ref{sec:conclusion} concludes the paper, along with remarks on possible extensions.

==> sections/results.tex <==
\section{Numerical Evaluation}
\label{sec:results}



The underlying use case analyzed in this work is the well-known CartPole problem, as implemented in the \emph{OpenAI Gym} library\footnote{\url{https://www.gymlibrary.dev/environments/classic_control/cart_pole/}}. In this problem, a pole is installed in a cart, and the task is to control the cart position and velocity to keep the pole in equilibrium. The physical state of the system is fully described by the cart position $x_t$ and velocity $\dot{x}_t$, and the pole angle $\psi_t$ and angular velocity $\dot{\psi}_t$. Consequently, the true state of the system is ${s_t = ( x_t, \dot{x}_t, \psi_t, \dot{\psi}_t )}$, and the semantic state space is $\mathcal{S}\subset\mathbb{R}^4$ (because of physical constraints, the range of each value does not actually span the whole real line).

At each step $t$, the observer senses the system by taking a color picture of the scene, which is in a space $\mc{P}=\left\{ 0, \dots, 255\right\}^{180 \times 360 \times 3}$. To take the temporal element into account, an observation $O_t$ includes two subsequent pictures, at times $t-1$ and $t$, so that the observation space is $\mc{O}=\mc{P}\times\mc{P}$. An example of the transmission process is given in Fig.~\ref{fig:cartpole}, which shows the original version sensed by the observer (above) and the reconstructed version at the receiver (below).

In the CartPole problem, the action space $\mathcal{A}$ contains just two actions $\mathtt{Left}$ and $\mathtt{Right}$, which push the cart to the left or to the right, respectively. At the end of each step, depending on the true state $s_t$, and on the taken action $a_t$, the environment will return a deterministic reward:
\begin{align}
    R_t = -x_{\text{max}}^{-1} |x_t|-\psi_{\text{max}}^{-1} |\psi_t|, \quad \forall t,
\end{align}
where $x_{\text{max}} = 4.8$ [m] and $\psi_{\text{max}} = 24^{\circ}$ [deg] are the maximal achievable values for the two quantities. The goal for the two agents is thus to maximize the cumulative discounted sum of the reward $R_t$, while limiting the communication cost.

\subsection{The Coding \& Decoding Functions}
\label{subsec:training_vqvae}


As mentioned in Section~\ref{subsec:coding}, the observer can optimize its coding function $\Lambda$ according to different criteria depending on the considered communication problem. However, as we explained in Section~\ref{sec:solution}, optimizing the choice of $\Lambda$ is usually not feasible due to the curse of dimensionality on the action space. Consequently, we rely on a pre-trained set $\mc{V}$ of \gls{vqvae} models, whose codebooks are optimized to solve the technical problem, i.e., minimizing the distortion on the observation measured using the \gls{mse}: $d_{A}(O, \hat{O}) = \text{MSE}(O, \hat{O})$. The training performance of the \gls{vqvae} with $N_{\Psi}=6$ is shown in Fig.~\ref{fig:vqvae_training}: the encoder converges to a good reconstruction performance, which can be measured by its \emph{perplexity}. The perplexity is simply $2^{H(p)}$, where $H(p)$ is the entropy of the codeword selection frequency, and a perplexity equal to the number of codewords is the theoretical limit, which is only reached if all codewords are selected with the same probability. The perplexity at convergence is 54.97, which is close to the theoretical limit for a real application.

\begin{figure}[t]
\centering
\includegraphics[width=0.8\columnwidth]{figures/cartpole}
\includegraphics[width=0.8\columnwidth]{figures/cartpole_tx}
\caption{Example of the original and reconstructed observation.}\vspace{-0.4cm}
\label{fig:cartpole}
\end{figure}

\begin{figure}[t]
\centering
\subfloat[PSNR.\label{fig:vqvae}]{\input{figures/training_vqvae}}%
\subfloat[Perplexity.\label{fig:perplexity}]{\input{figures/perplexity_vqvae}}%
\caption{Training of the \gls{vqvae} model with $N=6$.}\vspace{-0.4cm}
\label{fig:vqvae_training}
\end{figure}


The observer then uses \gls{drl} to foresightedly optimize the quantization level $\Psi_t$ at each time step, maximizing~\eqref{eq:varcapproblem} for each communication problem. We train the observer to solve the level-specific coding problem by designing three different rewards, depending on the considered communication level:
\begin{enumerate}
\item \emph{Level A (technical problem):} The reward for the observer is $r_t = \text{PSNR}(o_t, \hat{o_t}) - \beta \ell(m_t)$, where the \gls{psnr} is an image fidelity measure proportional to the logarithm of the normalized \gls{mse};
\item \emph{Level B (semantic problem):} The reward is $r_t = -\text{MSE}(s_t, \hat{s_t}) - \beta \ell(m_t)$, and the decoder needs to estimate the underlying physical state $s_t$ by minimizing the \gls{mse}, i.e., the distance between $s_t$ and $\hat{s}_t$ in the semantic space.  In our case, the estimator used to obtain $\hat{s}_t$ is a pre-trained supervised \gls{lstm} neural network;
\item \emph{Level C (effective problem):} In this case the reward is $r_t = Q(o_t,\pi(a_t|m_t)) - \beta\ell(m_t)$, where $Q(o_t, a_t)$ is the Q-function of the actor, measuring its long-term performance in the CartPole task when sampling actions $a_t$ according to its policy $\pi$ informed by the message $m_t$. The policy $\pi$ is given by a \gls{dqn} agent implementing an \gls{lstm} architecture, pre-trained using data with the highest available message quality (6 bits per feature). 
\end{enumerate}
We observe that, in this case, $i_{\mathcal{T}(s)} = s$, i.e., the task depends on all the semantic features contained in $s_t$. However, the $4$ values do not carry the same amount of information to the actor: depending on the system conditions, i.e., the state $s_t$, some pieces of information are more relevant than others.

\begin{figure*}[t]
\centering
    \subfloat{\input{figures/prob_legend}}\vspace{-0.2cm}\\
        \setcounter{subfigure}{0}
\subfloat[Technical problem.\label{fig:technical}]{\input{figures/tech_prob}}%
\subfloat[Semantic problem.\label{fig:semantic}]{\input{figures/sem_prob}}%
\subfloat[Effective problem.\label{fig:effective}]{\input{figures/eff_prob}}%
\caption{Performance of the communication schemes on the three levels of the remote \gls{pomdp}.}\vspace{-0.4cm}
\label{fig:performance}
\end{figure*}

\subsection{Results}
\label{subsec:results}

We assess the performance of the three different tasks in the CartPole scenario by simulation, measuring the results over 100 episodes after convergence. Fig.~\ref{fig:performance} shows the performance of the various schemes over the three problems, compared with a static \gls{vqvae} solution with a constant compression level. We trained the dynamic schemes with different levels of the communication cost $\beta$, so as to provide a full picture of the adaptation to the trade-off between performance and compression. We also introduce the notion of \emph{Pareto dominance}: if performance is an $n$-dimensional tuple $\eta=(\eta_1,\ldots,\eta_n)$, $\eta$ Pareto dominates $\eta'$ (which we denote as $\eta\succ \eta'$) if:
\begin{equation}
\eta\succ \eta' \iff \exists i:\eta_i>\eta_i' \wedge\eta_j\geq\eta_j'\,\forall j.
\end{equation}
We can extend this to the performance of schemes, which have multiple performance points. The definition of Pareto dominance for schemes $x$ and $y$ is: $x\succ y \iff \exists \eta_x\succ\eta_y\,\forall \eta_y.$
We consider the technical problem performance, shown in Fig.~\ref{fig:technical}: as expected, the Level A dynamic compression outperforms all other solutions, and its performance is Pareto dominant with respect to static compression. Interestingly, the Level B and Level C solutions perform worse than static compression: by concentrating on features in the semantic space or the task space, these solutions remove information that could be useful to reconstruct the full observation, but is meaningless for the specified task.

In the semantic problem, shown in Fig.~\ref{fig:semantic}, a lower \gls{mse} on the reconstructed state is better, and the Level B solution is Pareto dominant with respect to all others. The Level A solution also Pareto dominates static compression, while the Level C solution only outperforms it for higher compression levels, i.e., on the left side of the graph.

Finally, we consider the performance at the effectiveness level, shown in Fig.~\ref{fig:effective}: we can note that the performance in the task, summarized by the time that the cart-pole system is within the position and angle limits, is much higher for the Level C solution. Interestingly, however, it is not strictly Pareto dominant: for extreme compression levels, setting a static compression and retraining the actor to deal with the specific \gls{vqvae} used can provide a slight performance advantage. However, this is also a possibility for a Level C dynamic compression: retraining the actor to deal with the dynamically compressed messages could match the performance of the retrained static scheme, and in general, almost perfect control can be achieved with less than half of the average bitrate as the static compressor. We also note that in this case, the Level B solution performs worst: choosing the solution that minimizes the semantic distortion might not be matched to the task, as the state variables have equal weight, while a higher precision might be required when the quantization error might change the action the actor chooses.



%\begin{figure*}
%\input{figures/technical_frequencies.tex}
%\end{figure*}

%\begin{figure*}
%\input{figures/sematic_frequencies.tex}
%\end{figure*}



==> sections/solution.tex <==
\section{Proposed Solution}
\label{sec:solution}
 In this section, we introduce the architecture we used to represent $\Lambda$, the \gls{vqvae}, and discuss the remote \gls{pomdp} solution. As the \gls{vqvae} model is not adaptive, we consider an ensemble model with different quantization levels, limiting the choice of the observer to \emph{which} \gls{vqvae} model to use in the transmission. As the action space in~\eqref{eq:varcapproblem} is huge, techniques such as emergent communication that learn it explicitly are limited to very simple scenarios. By restricting the problem to a smaller action space, we may find a slightly suboptimal solution, but can deal with much more complex problems. 
 
\subsection{Deep VQ-VAE Encoding}
\label{subsec:vae}
In order to represent the encoding function $\Lambda$, and to restrict the problem in~\eqref{eq:varcapproblem} to a more manageable action space, the observer exploits the \gls{vqvae} architecture introduced in~\cite{van2017neural}. The \gls{vqvae} is built on top of the more common \gls{vae} model, with the additional feature of finding an optimal discrete representation of the latent space. The \gls{vae} is used to reduce the dimensionality of an input vector $X \in \mathbb{R}^I$, by mapping it into a stochastic latent representation $Z \in \mathbb{R}^L \sim q_{\phi}(Z | X)$, where $L < I$. The stochastic encoding function $q_{\phi}(Z | X)$ is a parameterized probability distribution represented by a neural network with parameter vector $\phi$. To find optimal latent representations $Z$, the \gls{vae} jointly optimizes a decoding function $p_{\theta}(\hat{X}|Z)$ that aims to reconstruct $X$ from a sample $\hat{X} \sim p_{\theta}(\hat{X} | Z)$. This way, the parameter vectors $\phi$ and $\theta$ are usually jointly optimized to minimize the distortion $d(X, \hat{X})$ between the input and its reconstruction, given the constraint on $Z$, while reducing the distance between $q_{\phi}(Z|X)$, and some prior $q(Z)$~\cite{vae2013} used to impose some structure or complexity budget. 

However, in practical scenarios, one needs to digitally encode the input $X$ into a discrete latent representation. To do this, the \gls{vqvae} quantizes the latent space by using $N$ $K$-dimensional codewords $z_1, \dots, z_N \in \mathbb{R}^K$, forming a dictionary with $N$ entries. Moreover, to better represent 3D inputs, the \gls{vqvae} quantizes the latent representation $Z$ using a set of $F$ codewords, each quantizing one feature $f(X)$ of the input, and chosen from a set of $N$ possible codewords. We denote the set containing the all $N^F$ codewords with $\mathcal{M}(N)$, as it represents the set of all possible messages the observer can use to convey to the actor the information on the observation $O$, by using $F$ discrete $N$-dimensional features. The peculiarity of the \gls{vqvae} architecture is that it jointly optimizes the codewords in $\mathcal{M}(N)$ together with the stochastic encoding and decoding functions $q_{\phi}$ and $p_{\theta}$, instead of simply applying fixed vector quantization on top of learned continuous latent variables $Z$. When the communication budget is fixed, i.e., constant value of $B$, the protocol to solve the remote \gls{pomdp} is rather simple: First, the observer trains the \gls{vqvae} with $N = 2^{\frac{B}{F}}$ to minimize the technical, semantic, or effective distortion $d_{\alpha}$, depending on the problem; Then, at each step $t$, the observer computes $\hat{m} \sim q_{\phi}(\cdot | o_t)$, and find $ m_t = \argmin_{m \in \mathcal{M}(N)} \| m - \hat{m} \|_2$.
The message $m_t$ is sent to the actor, which can optimize its decision on the action to take according to it.


\subsection{Dynamic Feature Compression}
\label{subsec:drl}


We can then consider the architecture shown in Fig.~\ref{fig:arch}, consisting of a set of \glspl{vqvae} $\mathcal{V} = \{ \Psi_1, \ldots, \Psi_V\}$, where each \gls{vqvae} has a different compression level $N_{\Psi}$: as we only consider the communication side of the problem, the actor is trained beforehand using the messages with the finest-grained quantization, which are compressed with the \gls{vqvae} $\Psi$ with larger value of $N$, i.e., larger codebook. 
 %with the highest $\Psi_v$. T
 The actor can then perform three different tasks, corresponding to the three communication problem: it can decode the observation (Level A) with the highest possible accuracy, using the decoder part of the \gls{vqvae} architecture, it can estimate the hidden state (Level B) using a supervised learning solution, or it can control the environment.


\begin{figure}
\centering
\input{figures/architecture}
\caption{Dynamic feature compression architecture.}\vspace{-0.4cm}
\label{fig:arch}
\end{figure}

In all three cases, the dynamic compression is performed by the observer, based on the feedback from the actor. The observer side of the remote \gls{pomdp}, whose reward is given in~\eqref{eq:varcapproblem}, is restricted to the choice of $\Psi_v$, i.e., to selecting one of the possible codebooks learned by each \gls{vqvae} in the ensemble model. Naturally, the feedback depends on the communication problem that the observer is trying to solve: at Levels A and B, the observer aims at minimizing distortion in the observation and semantic space, respectively, while at Level C, the objective is to maximize the reward of the actor.

In all three cases, \emph{memory} is important: representing snapshots of the physical system in consecutive instants, subsequent observations have high correlations, and the actor can glean a significant amount of information from past messages. This is a significant advantage of dynamic compression, as it can adapt messages to the estimated knowledge of the receiver.

However, the performance could still be improved: the observer is adapting its transmissions to the actor's task, but the actor's algorithms are fixed, while they could themselves be adapted to the dynamic compression strategy. This joint training is significantly more complex, and we consider it as a possible extension of the work.

==> sections/system_model.tex <==
\section{System Model}
\label{sec:system}

We consider a general model in which two agents cooperate to solve a \emph{remote \gls{pomdp}} problem. In the standard \gls{pomdp} formulation~\cite{pomdp}, one agent needs to optimally control a stochastic process defined by a tuple $\left< \mathcal{S}, \mathcal{A}, \Omega, P, O, R, \gamma\right>$, where $\mathcal{S}$ represents a set of system states, $\mathcal{A}$ is the set of feasible actions, and $\Omega$ is the observation set. The function $P : \mathcal{S} \times \mathcal{A} \rightarrow \Phi(\mathcal{S})$, where $\Phi(\cdot)$ represents all possible probability distributions over a set, gives the state transition probability, whose element $P_{ss'}^a$ provides the probability distribution of the next state $s' \in \mathcal{S}$ given that the system is in state $s \in \mathcal{S}$, and the agent has taken action $a \in \mathcal{A}$. On the other hand, $O : \mathcal{S} \rightarrow \Phi(\Omega)$ is an observation function, which provides the conditional probabilities $O(s, o) = Pr \left[ S_t = s | O_t = o\right]$, i.e., the probability that the system is in state $s$, given the observation $o$. Finally, $R: \mathcal{S} \times \mathcal{A} \rightarrow \mathbb{R}$ provides the average reward given to the agent when taking action $a$ in state $s$, denoted as $R_s^a$, and the scalar $\gamma \in [0, 1)$ is a discount factor.

Specifically, the \gls{pomdp} proceeds in discrete steps indexed by $t$, and at each step $t$ the agent can infer the system state $s_t$ only from the stochastic observation $o_t$, thus having partial information on it. Based on this observation, and on its policy $\pi : \Omega \rightarrow \Phi(\mathcal{A})$, which outputs a probability distribution over the action space for each possible observation, the agent interacts with the system by sampling an action ${a_t \sim \pi(a_t | o_t)}$. Then, given the real system state $s_t$ and the sampled action $a_t$, the agent receives a feedback from the system in the form of a reward ${r_t = R_{s_t}^{a_t}}$. The goal for the agent is to optimize its policy $\pi$ to maximize the expected cumulative reward discounted reward $G = \mathbb{E}\Big[ \sum_{t} \gamma^t r_t \Big]$. We can see that the \gls{pomdp} is indeed built on top of the \gls{mdp} formulation, with the addition of noisy observations.

\subsection{The Remote POMDP}

In this paper we consider a variant of the \gls{pomdp}, that we define \emph{remote \gls{pomdp}}, in which two agents are involved in the process. The first agent,  i.e., the \emph{observer}, receives the observation $o_t \in \Omega$, and needs to convey such information to a second agent, i.e., the \emph{actor}, through a constrained communication channel, which limits the number of bits the observer can send. The actor then chooses and takes an action. Consequently, the amount of information the observer can send to the actor is limited. This system can formalize many control problems in future \gls{iiot} systems, as sensors and actuators can potentially be geographically distributed, and the amount of information they can exchange to accomplish a task is limited due to the shared wireless medium, which has to be allocated to the large amount of devices installed in the factory, as well as by the energy limitations on the sensors.

% ------------------------- %

In order to transmit the most relevant information to the actor, the observer chooses its transmission $m_t \in \mathcal{M}$, where $\mathcal{M}$ is the set of possible messages (which corresponds to the observer's action space). Then, based on the received message $m_t$, the actor optimizes its own policy $\pi^a(a_t | m_t)$ to maximize $G$, and to optimally solve the underlying control problem. As the objective of the observer is to minimize channel usage, i.e., communicate as few bits as possible, while maintaining the highest possible performance in the control task, we consider the problem of adaptive encoding.

In order to solve this problem, the observer needs to have a way to gauge the \emph{value} of information, as described in the introduction: information theory, and in particular rate-distortion theory, have provided the fundamental limits when optimizing for the technical problem, i.e., Level A, where the goal is to reconstruct the source signals with the highest fidelity~\cite{cover:IT}. The first and simplest way to solve the remote \gls{pomdp} problem is to blindly apply standard rate-distortion metrics to compress the sensor observations into messages to be sent to the agent. The observer's policy is then independent from the actor's task, and can be computed separately. 

However, in robotics and remote control applications, which are the targets of our analysis, the receiver is only interested in the part of the message conveying relevant information on the underlying physical system, or on the task to be accomplished, and so further source redundancy may be exploited to reduce the size of the message. Consequently, it is natural to assume that the observations convey some sort of physical information on the underlying process to be controlled. A natural projection of the raw observations into a semantic space can be assumed, which captures the physical meaning contained in the observed signals, removing meaningless information due to noise and/or sensor additional data.

As an example, in the CartPole problem analyzed in this work (see Section~\ref{sec:results}), one sensor observation is given by two consecutive 2D camera acquisitions, which only implicitly capture the needed physical system information, e.g., the angular position and velocity of the pole. By employing semantic source coding, the sensor can extract the underlying physical quantities from the raw observations, which can be useful for multiple applications at the receiver, considering not reconstruction accuracy but rather semantic fidelity, which measures the error on the underlying physical values rather than on the raw sensory observation, thus solving the Level B communication problem. What can be gained with the semantic formulation in terms of trade-off between size of the message, and performance on the downstream task at the receiver, with respect to the Level A system is the second question we try to answer with our analysis. 

Going further, one may only want to convey the physical information related to a specific task, constructing a Level C system as envisioned in~\cite{shannon1949mathematical}. For this purpose, the sensor has access to feedback signals indicating the quality of the actions of the remote agent when decoding specific messages. This data can be used by the sensor to adjust the observations coding scheme to optimally trade off size of the message, and performance of the remote agent on the specific control problem. How to design this scheme, and how this scheme compares with Level A and B designed systems, are the other questions we answer with our study.

\subsection{The Information Bottleneck}
\label{subsec:info_bottleneck}
We now consider the observer's encoding function. As the actor can use the received message $m_t$, along with its memory of past messages at previous steps, to choose an action $a_t$, the encoding function is $\Lambda: \Omega\times\mc{M}^{\tau} \rightarrow \mc{M}$, which considers a case with memory $\tau$. The function will generate a message $M_t = \Lambda(O_t,M_{t-\tau},\ldots,M_{t-1})$ to be sent to the actor at each step $t$. As mentioned above, the encoding function $\Lambda$ can be optimized to solve one of the three communication problems.

We assume that the underlying state of the physical system at time $t$ can be entirely described by the variable $s_t$, which is an element of the physical state space $\mc{S}$. However, in our remote \gls{pomdp} formulation, the sensor can access to this state only through the observation $o_t$, which is in general a stochastic function of $s_t$ whose codomain is the observation space $\Omega$. In addition to this, we assume that the performance at time $t$ in a particular task $\mc{T}$ 
%(i.e., the parameter that the two agents aim to maximize) 
depends only on a sufficient statistic $i_{\mc{T}}(s_t)$ of the state. Denoting the number of bits required to represent the random variable $X$~\cite{cover:IT} as $b(X)$, we assume that 
\begin{align}
\label{eq:relation}
    b(i_{\mc{T}}(S)) < b(S) < b(O) \quad \forall S \in \mc{S}.
\end{align}
We implicitly impose a Markov Chain structure ${i_{\mc{T}}(S) \rightarrow S \rightarrow O}$. The random quantity $i_{\mc{T}}(S)$ represents the minimal description of the system with respect to the task $\mc{T}$, i.e., no additional data computed from $s_t$ adds meaningful information for the actor when solving $\mc{T}$. The state $S$ may also include task-irrelevant physical information on the system. However, both $S$ and $i_{\mc{T}}(S)$ are unknown quantities, as the observer only receives a noisy and high-dimensional representation of $S$ through $O$. This is a well-known issue in \gls{drl}: in the original paper presenting the \gls{dqn} architecture~\cite{mnih2015human}, the agent could only observe the screen while playing classic arcade videogames, and did not have access to the much more compact and precise internal state representation of the game. Introducing communication and dynamic encoding adds another layer of complexity to the problem.

\subsection{Encoding and Distortion}\label{subsec:coding}
In our remote \gls{pomdp}, the communication channel between the sensor and the actor is not ideal, thus the information the observer can convey to the actor at each step $t$ is limited to a maximum number of bits $B$ per message. Consequently, the problem introduces an information bottleneck between the observation $o_t$ and the final action $a_t$ the actor can take, which is based on the message $M_t$ conveyed through the channel. In principle, whenever $b(O)>B$, the constrained communication introduces a distortion $d(O, \hat{O})$, whose theoretical asymptotic limits are given by rate-distortion theory~\cite{cover:IT}. If we also consider \emph{memory}, i.e., use past messages in the estimation of $\hat{O}$, the mutual information between $O$ and previous messages can be used to reduce the distortion, improving the quality of the estimate.
In the semantic problem, the aim is to extrapolate the real physical state of the system $s_t$ from the observation $o_t$, which can be a complex stochastic function. In general, the real state lays in a low-dimensional semantic space $\mc{S}$. The term semantic is motivated by fact that, in this case, the observer is not just transmitting pure sensory data, but some meaningful physical information about the system. Consequently, the distortion to be considered in the trade-off is in the semantic space $d(S_t, \hat{S}_t)$, where the estimation $\hat{S}_t$ is performed by the actor based on its knowledge of the message, as well as its memory of past messages. To be even more efficient and specific with respect to the task $\mc{T}$, the observer may optimize the message $M_t$ to minimize the distortion 
%$d(i_{\mc{T}}(S_t)|M_{t-\tau},\ldots,M_t)$ 
between the effective representation $i_{\mc{T}}(s_t)$, which contains only the task-specific information, and the knowledge available to the actor. Naturally, any $M_t\in\mc{M}$ must be at most $B$ bits long, in order to respect the constraint. If we define a generic distortion 
%$d_{\alpha}(S_t,M_t)$,
$d_{\alpha}$ between the real quantity and its reconstruction at the different levels, which are indexed by $\alpha\in\{A,B,C\}$, the observer's task %\gls{pomdp} 
is then defined as follows:
\begin{equation}
\Lambda^*=\argmax_{\mathclap{\Lambda:\Omega\times\mc{M}^{\tau}\rightarrow\mc{M}}}\E{\sum_{t=0}^\infty \gamma^t\left[d_{\alpha} -\beta\ell(M_t)\right]\bigg| S_0,\Lambda},\label{eq:varcapproblem}
\end{equation}
where $\beta\geq0$ is a communication cost parameter and the function $\ell(\cdot)$ represents the length (in bits) of a message. The observation space of the observer is given by $\Omega\times\mc{M}^{\tau}$, while the observation space of the actor is $\mc{M}^{\tau+1}$, as it only receives the messages from the observer.
